Event generation with Sherpa 3

Sherpa is a general-purpose Monte Carlo event generator for the simulation of particle collisions in high-energy collider experiments. We summarise new developments, essential features, and ongoing improvements within the Sherpa 3 release series. Physics improvements include higher-order electroweak corrections, simulations of photoproduction and hard diffraction at NLO QCD, heavy-flavour matching in NLO multijet merging, spin-polarised cross section calculations, and a new model of colour reconnections. In addition, the modelling of hadronisation, the underlying event and QED effects in both production and decay has been improved, and the overall event generation efficiency has been enhanced.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}

\usepackage{axodraw}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{graphicx}
\usepackage{setspace}
\usepackage{threeparttable}
\usepackage{relsize}
\usepackage{ifthen}
\usepackage{lineno}
\usepackage{enumerate}
\usepackage{makeidx}
\usepackage{showidx}

\setlength{\parindent}{0.0in}
\setlength{\parskip}{0.0in}

%%% Structuring
\newcommand{\Vp}{\ensuremath{\vphantom{\frac{|^|}{|^|}}}}
\newcommand{\LINE}{\underline{\hspace*{13.5cm}\hphantom{t}}\\}
\newcommand{\comment}[2][]{\noindent\LINE{\bf{#1}: }{#2}\\\LINE}
%\newcommand{\todo}[1]{\textbf{\color{red}#1}}
%\newcommand{\didit}[1]{\textbf{\color{blue}did it (#1)}}
%\newcommand{\checked}[1]{\hfill{\textbf{\color{green}\checkmark(#1)}}}
\newcommand{\todo}[1]{\fbox{\begin{minipage}{\textwidth}\textbf{#1}\end{minipage}}}
\newcommand{\didit}[1]{\textbf{\underline{#1}}}
\newcommand{\checked}[1]{\hfill{\textbf{\underline{#1}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Maths macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_maths}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Physics macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_physics}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Section references
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_refs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Experiments / Machines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_collabs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Software names
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros_codes}





==> text/cr.tex <==
\subsubsection{Colour reconnections}
\label{sec:sherpa:had:colrec}

The partons produced by the hard and multiple parton interactions, their
subsequent parton showers and the break-ups of the beam remnants turn into
primary hadrons. These primary hadrons have their colours assigned in the large-$N_c$ limit.
This means that effectively, at this stage, every colour in the parton
ensemble has exactly one anti-colour and vice versa.  The difference between
the $N_c\to\infty$ approximation and the actual value $N_c=3$ and the
existence of potential soft non-perturbative gluon interactions (so-called
``gluers''~\cite{Dokshitzer:1991wu}) suggests that the original colour
assignments of the partons may undergo a rearrangement.  In particular
the non-perturbative nature of the long-range strong interactions introduces
significant liberty in the modelling of such colour reconnections (CRs).

%In \Pythia's original CR model, introduced in~\cite{Sjostrand:1987su}, the
%colour strings of multiple parton scatters and beam remnants are re-arranged
%in such a way that the overall length of the string,
%$\lambda\approx\sum_{\langle ij\rangle}\log\frac{m^2_{ij}}{s_0}$ is minimised,
%where $\langle ij\rangle$ denotes pairs of colour-connected partons in the
%$N_c\to\infty$ limits and $s_0$ is a parameter with values around 1 GeV$^2$. This
%original idea and its realisation have been further refined, for example
%in~\cite{Skands:2007zg}, where shortest overall string lengths are identified
%with a simple version of an annealing algorithm.

%Driven by the analysis of fully hadronically decaying $W$-pairs at \LEP,
%perturbative considerations on the interference of gluon emissions by the
%two $q\bar{q}$ pairs formed in the decays of the two $W$ bosons improved
%the understanding of a reconnection probability as a colour-suppressed effect,
%and an analysis of the space-time picture of the hadronisation of the parton
%ensemble, led to an extension of the original model including
%``finite-distance'' effects~\cite{Sjostrand:1993hi,Khoze:1994fu,Khoze:1999up},
%with ideas borrowed from the similarity of super-conductivity and the
%formation of strings that resemble the linear QCD potential at large
%distances.  Space-time considerations, which are more relevant in heavy ion
%collisions were recently worked out within \Pythia in~\cite{Lonnblad:2023stc}.

%The original \Pythia model was extended in~\cite{Sjostrand:2004pf} by a more
%detailed treatment of the interplay of MPIs, beam remnants and the transport
%of baryon number through suitably defined ``junctions''.

%Similar ideas, but in the framework of the cluster hadronisation model, were
%also the basis for the colour reconnection model in \Herwig, with the
%string length replaced by the cluster masses. In the original model
%formulation of~\cite{Webber:1997iw}, a ``colour swap'' between two clusters
%did happen with a probability of 1/9, if the resulting clusters have a
%reduced mass. In~\cite{Gieseke:2012ft} the original model was modified such
%that cluster configurations with the smallest overall summed mass,
%$\lambda = \sum_{\langle ij\rangle}m_{\langle ij\rangle}^2$, with the summation
%running over all clusters $\langle ij\rangle$, is found in a simulated
%annealing procedure.

%Expanding on ideas how colour evolves through soft gluon emissions below the
%parton shower's infrared cut-off, the interplay of CRs and baryon production
%was further analysed in~\cite{Gieseke:2017clv,Gieseke:2018gff}, and space-time
%considerations were included in \Herwig's CR model in~\cite{Bellm:2019wrh}.
%These ideas are continuously developed, see {\textit{e.g.}}~\cite{Platzer:2022jny},
%which discusses the interface of correct colour evolution at amplitude level,
%\ie with interferences, and the hadronisation.

The model in \Sherpa incorporates various ideas from earlier literature~\cite{
  Sjostrand:1987su,Skands:2007zg,Sjostrand:1993hi,Khoze:1994fu,Khoze:1999up,
  Lonnblad:2023stc,Sjostrand:2004pf,Webber:1997iw,Gieseke:2012ft,
  Gieseke:2017clv,Gieseke:2018gff,Bellm:2019wrh,Platzer:2022jny}.  Assuming
that $N$ different colours (matched by exactly $N$ anti-colours) emerge from
the scatters, showers, and beam remnants, the model checks $N^2$ times for
possible colour reassignments. In each such attempt two colours $i$ and $j$
are randomly chosen, and the relative distances $d$ of the corresponding
parton pairs $\langle i\bar{i}\rangle$ and $\langle j\bar{j}\rangle$ and the
possibly swapped pairs $\langle i\bar{j}\rangle$ and $\langle j\bar{i}\rangle$
is calculated. For each pair $kl$ the distance in momentum space is given by
\begin{equation}
  d_{kl} = \log\left(1+\frac{p_kp_l-m_km_l}{Q_0^2}\right)\,,
\end{equation}
possibly multiplied with factors representing distances in space-time between
the partons. Based on this distance, a colour re-assignment happens with a
probability given by
\begin{equation}
  P_{\mathrm{swap}}(i\leftrightarrow j) = R_c\cdot\left\{1-\exp\left[\eta\,
    \left(d_{i\bar{i}}+d_{j\bar{j}}-d_{i\bar{j}}-d_{j\bar{i}}\right)
    \right]\right\}\,.
\end{equation}
In the equations above, $Q_0$, $R$ and $\eta_q$ are parameters, with (untuned)
defaults for the infrared scale in the distance measure $Q_0\approx 1$ GeV,
$R_c\approx 1/9$ for the colour factor and $\eta_Q\approx 0.1$ for the weight
of the distances in the exponential.


==> text/had.tex <==
\subsubsection{Cluster hadronisation}
\label{sec:sherpa:had:cluster}

\Sherpa's default hadronisation model~\cite{Winter:2003tt,Chahal:2022rid}
is based on the twin concepts of local parton-hadron duality (LPHD)~\cite{Azimov:1984np}
and preconfinement~\cite{Amati:1979fg,Bassetto:1979vy,Marchesini:1980cr},
which postulate that the flow of quantum numbers, momenta, and energies at
the hadron level closely follows their counterparts at the parton level, and
that the transition from partons to hadrons proceeds through the formation
of colourless clusters with a {\em perturbatively} calculable mass spectrum.
The first realisation of the LPHD paradigm in the form of the Feynman--Field
independent fragmentation model~\cite{Field:1977fa} suffered from a range of
theoretical issues, among them lack of Lorentz invariance. These issues where
ultimately resolved by the inclusion of the preconfinement idea which
introduced the intermediate step of a non-perturbative splitting of gluons
into quark--\-anti-quark pairs~\cite{Hoyer:1979ta,Ali:1979em} and the
subsequent formation of colour-neutral clusters and their decay into
hadrons~\cite{Field:1982dg}.  The first cluster fragmentation model embedded
in a widely used event generator, \Herwig~\cite{Corcella:2000bw,Bewick:2023tfi},
was introduced shortly afterwards~\cite{Marchesini:1983bm,Webber:1983if}
and is continuously improved~\cite{Bellm:2015jjp,Masouminia:2023zhb,Hoang:2024zwl}.
%This includes, for example, improvements in capturing spin
%effects in fragmentation and decay of heavy quarks~\cite{Masouminia:2023zhb},
%and studies to highlight the interplay of the infrared parton shower cut-off
%with hadronisation and the redefinition of kinematics in the fission of
%heavy primary clusters into lighter secondary ones~\cite{Hoang:2024zwl}.

\Sherpa's cluster model~\cite{Winter:2003tt,Chahal:2022rid}
differs from the \Herwig model in multiple ways.
Firstly, \Sherpa does not introduce non-perturbative gluon masses but rather
keeps the gluons massless, and, if kinematically viable, allows not only light up and down quarks,
but also strange quarks and diquarks as decay products of their forced splitting
at the onset of hadronisation. This results in the presence of baryonic
clusters throughout the hadronisation stage.  Secondly, the fission of
relatively heavy clusters into two lighter ones is not parametrised by
selecting masses of the latter in typically isotropic decays.  Instead,
\Sherpa distributes light-cone momentum fractions of the new clusters with
respect to the constituents of the decaying cluster according to
``fragmentation functions'', and adds a Gaussian distributed transverse
momentum to the decay kinematics. Finally, there are also differences in
the treatment of binary cluster decays into primary hadrons, including
kinematics and the way the hadron species are selected. Overall, despite the footing
of both models in the same underlying physics assumptions, these differences
result in two manifestly different hadronisation models with different sets of critical
parameters that need to be tuned to data.

\subsubsection[Interface to \Pythia]{Alternative hadronisation model via interface to Pythia 8}
\label{sec:sherpa:had:lund}

An alternative approach to hadronisation is provided by the string picture
of QCD~\cite{Artru:1974hr,Bowler:1981sb,Andersson:1983ia} which builds on
the observation of a potential between colour charges that increases
linearly with their position-space distance\footnote{
Approaches to combine the respective benefits of string and cluster
hadronisation~\cite{Gottschalk:1983fm,Gottschalk:1986bv} have not been
followed up in the past decades, arguably because they have not been provided
in the form of a widely used event generator.}.
The potential is represented by one-dimensional strings, which carry a finite
energy density per unit length.  As the strings are ``stretched'' with the
partons moving away from each other, their stored energy allows the dynamic
creation of quark--\-anti-quark pairs, akin to the Schwinger mechanism in
QED~\cite{Sauter:1931zz,Schwinger:1951nm}, essentially breaking the string into smaller,
\ie lighter fragments.  Successive refinements, including, among
others, symmetrising the string fragmentation function whilst respecting
Lorentz-invariance and causality~\cite{Andersson:1983jt}, extending the model
beyond the simple case of strings spanned by quark--\-anti-quark pairs and
including the effect of gluons~\cite{Andersson:1979ij,Sjostrand:1984ic}, and
the modelling of baryon production~\cite{Andersson:1981ce} have contributed
to establishing the Lund model~\cite{Sjostrand:1982fn,Andersson:1997xwk} as
the phenomenologically probably most successful hadronisation model.  Recent
developments include aspects relevant for the modelling of fragmentation in
dense QCD environments~\cite{Bierlich:2020naj,Bierlich:2022oja}, the
modelling of spin effects~\cite{Kerbizi:2021pzn} or hyper-fine splitting
between quark and hadron masses~\cite{Bierlich:2022vdf} in fragmentation.

\Sherpa provides an interface to the Lund model implemented in
\Pythia8~\cite{Sjostrand:2006za,Bierlich:2022pfr}, see App.~\ref{app:install} for instructions of how to enable it.
The support for both cluster hadronisation and String fragmentation available in \Sherpa,
allows for direct comparisons of hadronisation models and their observable effects
by having an identical treatment of the perturbative phase of the event evolution.


==> text/nlo.tex <==



==> text/nnlo.tex <==
\subsubsection{Hard scatterings at \texorpdfstring{\NNLO}{NNLO} accuracy}
\label{sec:sherpa:me:nnlo}
0.5 pages NNLO QCD -- SH


==> text/pols.tex <==
\subsubsection{Cross sections for polarised lepton beams}
\label{sec:dec:beampol}
At purposed lepton-collider experiments, the ability to polarise the 
incoming beams can be used to enhance the signal rates considerably
while also suppressing unwanted background processes. In annihilation
processes the helicity of incoming particles
are correlated with their spin and therefore can be tuned to suppress or
enhance various Standard Model processes. In the case of scattering 
processes the helicities of the initial-state leptons are directly
related to the properties of any produced particles. By varying the
polarisations of the incoming beams properties
of these particles such as their chiral couplings and quantum numbers
 can be probed~\cite{Moortgat-Pick:2005jsx}. 

In \Sherpa, it is possible to simulate events with longitudinally-polarised 
beams by reweighting the helicity amplitudes with the corresponding fractional
polarisation ($P_{e^\pm})$ using the \Amegic matrix element generator. This can
be combined with a YFS resummation, as described in \SecRef{sec:sherpa:yfs:ee},
to further improve the accuracy of the simulation for linear colliders. Since
YFS resummation is based on the soft limit, the matching of higher-order corrections with
beam polarisation can be achieved and will allow \Sherpa to provide NLO EW accurate
predictions. For example, in Tab.~\ref{table:cross_sections} we illustrate the
effect of beam polarisation on the Higgstrahlung process. Due to the chiral couplings
of the weak current polarised initial states can result in significant
enhancements to the WW fusion channel.

% \begin{align}
% \sigma_{P_{e^-},P_{e^+}} &= \frac{1}{4}\left((1+P_{e^-})(1+P_{e^+})\sigma_{RR} + (1-P_{e^-})(1-P_{e^+})\sigma_{LL} \right. \nonumber \\
% &\quad \left. + (1+P_{e^-})(1-P_{e^+})\sigma_{RL} + (1-P_{e^-})(1+P_{e^+})\sigma_{LR}\right)
% \label{EQ:PolXS}
% \end{align}

\begin{table}[ht]
	\centering
	\begin{tabular}{c| c c c}
		$(P_{e^-}, P_{e^+})$ & $HZ$ & $H\nu_e\bar{\nu}_e$ & $He^+e^-$ \\
		\hline
		\hline
		(0, 0)       & 1.00 & 1.00 & 1.00 \\
		(-0.8, 0)    & 1.17 & 1.68 & 1.19 \\
		(-0.8, 0.3)  & 1.47 & 2.18 & 1.50 \\
		(-0.8, -0.3) & 0.87 & 1.19 & 0.88 \\
		(0.8, 0.0)   & 0.83 & 0.32 & 0.83 \\
		(0.8, 0.3)   & 0.65 & 0.34 & 0.65 \\
		(0.8, -0.3)  & 1.00 & 0.31 & 1.00 \\
		\hline
	\end{tabular}
	\caption[width=0.85\textwidth]{Total cross sections for $e^+e^-\rightarrow X$ normalised
        to the unpolarised result for different initial-state polarisation combinations at \sqrts=380\,\UGeV.}
	\label{table:cross_sections}
\end{table}


\subsubsection{Cross sections for polarised intermediate gauge bosons}
\label{sec:dec:pols}
% Add one engaging sentence explaining the importance and current interest in polarisation
Vector boson polarisation measurements very recently started to become an extensive studied field, mainly due to the direct connection of the longitudinal polarisation state to the electroweak symmetry breaking mechanism. Strategies in LHC Run 2 \& 3 for measuring the polarisation are based on fully exclusive events for polarised cross sections from Monte Carlo event generators used as fitting templates to extract polarisation information from the measurable unpolarised distributions. With this release, the ability of \Sherpa simulating polarised cross sections for intermediate vector bosons is added \cite{Hoppe:2023uux}. Different to other tools, calculating polarisation templates for each polarisation state separately \cite{Ballestrero:2007xq, Ballestrero:2017bxn, BuarqueFranzosi:2019boy, Javurkova:2024bwa, Pelliccioli:2023zpd}, \Sherpa provides event-wise fully differential polarisation fractions on top of an unpolarised simulation in narrow-width approximation, added as additional event weights. Those fractions are calculated based on the complete helicity-dependent amplitude tensor such that also interferences between different polarisations are accessible on an event-by-event basis. Various reference systems can be investigated, even within a single simulation run. The polarisation framework is build upon \Sherpa's decay suite for unstable particles, hence a more detailed description of the on-shell approximation used for the polarisation definition can be found in \SecRef{sec:sherpa:me:dec}. 

The simulation of polarisation effects is not limited to LO, also approximate NLO QCD effects matched to parton shower via \Sherpa's MC@NLO and multi-leg merging (see \SecRef{sec:sherpa:mm:mcnlo} and \SecRef{sec:sherpa:mm:mets}) are available, the former for the first time at all. Within the approximate NLO QCD calculation, dubbed nLO QCD, polarisation fractions are calculated differently based on the event type in the MC@NLO formalism. For $\boldsymbol{\mathbb{H}}$ and resolved $\boldsymbol{\mathbb{S}}$ events, the corresponding amplitude tensor is constructed using the complete real emission amplitude. Hence, the correct polarisation fractions, up to NLO QCD, are used for both soft and hard emissions. For unresolved $\boldsymbol{\mathbb{S}}$ events, however, the amplitude tensor is solely build using the Born expression, i.e. all virtual and ultra-soft and/or -collinear emission corrections are neglected. As the number of events in this category is generally small, and this construction is only used to determine the polarisation fractions in the otherwise fully NLO QCD-accurate unpolarised sample, the error introduced in this way is expected to be small. 

In Fig.~\ref{fig:pols:nLOPS}, the nLO QCD+PS contribution to polarised, inclusive $\text{W}^+$Z production for the lepton rapidity in the laboratory frame is shown as an example. It illustrates the importance of higher order QCD effects included in polarisation templates since they can be very large and non-trivial. Comparisons with complete NLO QCD fixed order calculations confirmed that our nLO QCD approximation can reproduce all main contributions of the full calculation since they are strongly dominated by real corrections. Hence, also  multi-leg merged calculations are able to describe the bulk of the NLO QCD effects, if small merging scales are used, as demonstrated in Fig.~\ref{fig:pols:merging}. 
\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{plots/Polarisation_VB/WZ_eta_WLep_Lab.pdf}
	\caption{Double-polarised distributions of the positron rapidity $y_{e^+}$ in inclusive W+Z production at nLO+PS (polarised distribution)	/ NLO+PS (unpol, full) accuracy; polarisation states are defined in the laboratory (Lab). K-factors (bottom panel) are the ratio of n(N)LO+PS over LO+PS cross sections. All \Sherpa distributions agree well with MOCANLO+COLLIER+RECOLA complete NLO QCD fixed-order predictions in~\cite{Denner:2020eck}, Fig. 1 and 3. In addition, the interference contribution is shown. Figure adapted from \cite{Hoppe:2023uux}.}	
	\label{fig:pols:nLOPS}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.85\textwidth]{plots/Polarisation_VB/WZ_merging_NLOtoLO_COM.png}
	\caption{Integrated polarisation fractions for inclusive $\text{W}^+$Z boson production at the LHC (13~TeV) for LO+1j simulations matched to parton shower using different merging scales. For comparison, also polarisation fractions at nLO+PS and LO+PS are shown. The polarisation is defined in the $\text{W}^+$Z boson centre-of-mass frame. Figure adapted from \cite{Hoppe:2023uux}.}	
	\label{fig:pols:merging}
\end{figure}

Extensions to full NLO QCD and approximate NLO EW as well as external polarisations are foreseen for future releases.       


==> text/remnants.tex <==
\subsubsection{Beam remnant handling}
\label{sec:sherpa:had:beamremnant}
In collisions involving hadronic initial states, typically one or more partons
are extracted from the incoming beam particles through the perturbatively
described signal processes and the perturbatively modelled multi-parton
interactions (see Sec.~\ref{sec:sherpa:mi}).
Both types of perturbative calculations are dressed with parton
showers (see Sec.~\ref{sec:sherpa:showers}), which ultimately terminate at low
transverse-momentum scales of around 1 GeV.

In \Sherpa, the breakup of incoming hadrons and the formation of the beam
remnants at this point is modelled after all MPI and associated parton showering
steps have terminated and a list of shower initiators can be extracted
from the incoming hadron. The physics model is the following:
\begin{enumerate}
\item Flavour compensation: assuming an incoming hadron to consist of a
      valence quark--diquark pair, and that di-quarks cannot act as shower
      initiators, the flavours of the shower initiators have to be compensated.
      One of them may be a valence quark -- shower initiators are assigned as
      valence quarks with a probability obtained from the PDFs at the lowest
      scale.  All other ``net'' quark flavours among the shower initiators
      are compensated with a corresponding anti-flavour spectator.
\item Colour compensation: as the overall hadron must form a singlet, \Sherpa
      assumes a colour-ordered list of partons of the type $q-g-g-\dots-(qq)$,
      where $q$ and $(qq)$ denote the valence quark and diquark.  The model
      also assumes that flavour--anti-flavour pairs, either formed by
      the shower initiators of independent MPI scatters or by compensating
      individual flavours with a corresponding anti-flavour spectator,
      emerge from a gluon and therefore will be in a relative colour-octet
      state.
\item Longitudinal momenta: The longitudinal momenta of the shower initiators
      are already fixed, and those for the spectators in the beam breakup
      are selected according to the PDFs.  The longitudinal momentum for the
      valence diquark is given by the residual at the end of the process.
\item Transverse momentum: \Sherpa models the finite ``intrinsic'' transverse
      momentum $k_\perp$ inside the hadrons, akin to Fermi motion by
      assuming a Gaussian distribution, cut-off at large values through a
      polynomial,
      \begin{equation}
      \mathcal{P}(k_\perp)\propto
      \exp(-(k_\perp-k_{\perp,0})^2/\sigma^2) (k_{\perp, \text{max}}-k_\perp)^\eta\,.
      \end{equation}
      The parameters of this distribution depend on the hadron forming the
      beam and scale with the center-of-mass energy of the collision.
      \Sherpa allows different parameter values for parton-shower initiators
      and the spectator.
\item Overall momentum conservation:  To ensure overall momentum
      conservation after assigning individual intrinsic transverse momenta
      for the partons, \Sherpa allows two recoil strategies, which
      slightly modify both transverse and longitudinal momenta.  In a
      ``democratic approach'' the overall excess transverse momentum is
      compensated by subtracting it from the partons in proportion to their
      longitudinal momenta.  Alternatively, \Sherpa compensates in a similar
      fashion, the recoil of the shower initiators with the spectators and
      vice versa.  This leaves the question of overall momentum
      conservation within the beam break-up, as in most cases the combined
      invariant mass of partons coming from a hadron differs from its mass.
      In hadron-hadron collisions this is achieved by shuffling momenta
      between the two hadrons, while in collisions involving only one
      incident hadron, this compensation happens between initial and
      strongly interacting final states.
\end{enumerate}

